ShadowGenes: Leveraging Recurring Patterns within Computational Graphs for Model Genealogy

Machine learning model genealogy enables practitioners to determine which architectural family a neural network belongs to. In this paper, we introduce ShadowGenes, a novel, signature-based method for identifying a given model's architecture, type, and family. Our method involves building a computational graph of the model that is agnostic of its serialization format, then analyzing its internal operations to identify unique patterns, and finally building and refining signatures based on these. We highlight important workings of the underlying engine and demonstrate the technique used to construct a signature and scan a given model. This approach to model genealogy can be applied to model files without the need for additional external information. We test ShadowGenes on a labeled dataset of over 1,400 models and achieve a mean true positive rate of 97.49% and a precision score of 99.51%; which validates the technique as a practical method for model genealogy. This enables practitioners to understand the use cases of a given model, the internal computational process, and identify possible security risks, such as the potential for model backdooring.

==> sections/scratch.tex <==
Both of the previously described subgraphs were observed in the GerNet (GE-Net) model, which was a GPU-Efficient version of ResNet. The subgraphs containing these blocks are highlighted in Figure 6. 

\begin{figure}[H] 
    \centering
    \includegraphics[scale=0.58]{images/gernet_resnet_sig_neato.png}
    \caption{The identifiable repeating patterns found in ResNet models as observed in GerNet models. The edges colored red depict the use of the '*' value in the signature.}
    \label{fig:example}
\end{figure}

BoTNet was built on top of a ResNet architecture backbone while replacing the later convolutional layers with a global self-attention mechanism. This is shown in Figure 7. 

\begin{figure}[H] 
    \centering
    \includegraphics[scale=0.5]{images/botnet_neato.png}
    \caption{The identifiable repeating patterns found in ResNet models as observed in BoTNet models, with the start of the self-attention layer included.}
    \label{fig:example}
\end{figure}


\subsection{Recognizing Components of Architectures}

we can tell that it is transformers, we look at the attention mechanism and stuff like that and can tell that a specific part is the attention mechanism of model X or Y. this then helps us tell what the task is

\subsection{Using Signatures to Trace Model Genealogy of Unknown Model Architectures}

Camembert is just roberta


\begin{longtable}{|c|c|}
\hline
Model Class & Percentage Accuracy \\ \hline
\endfirsthead
% \hline
% Model Class & Percentage Accuracy \\ \hline
% \endhead
\endfoot
\hline
\endlastfoot
% Table content here
        AlexNet & 100\% \\
        BEIT & 100\% \\
        BERT & 100\% \\
        BigBird & 100\% \\
        BoTNet & 100\% \\
        CAIT & 100\% \\
        CoaT & 100\% \\
        ConVit & 100\% \\
        ConvBERT & 100\% \\
        ConvMixer & 100\% \\
        ConvNeXt & 88.46\% \\
        CrossVit & 100\% \\
        CspNet & 100\% \\
        DEIT3 & 100\% \\
        DLA & 100\% \\
        DPN & 80.0\% \\
        DarkNet & 100\% \\
        DeBERTa & 100\% \\
        DenseNet & 86.36\% \\
        DistilBERT & 100\% \\
        ECA-ResNet & 100\% \\
        EdgeNeXt & 100\% \\
        EfficientNet & 81.33\% \\
        ELECTRA & 100\% \\
        GcResNet & 100\% \\
        GcResNext & 100\% \\
        GerNet & 100\% \\
        GoogLeNet & 100\% \\
        HighResolutionNet & 100\% \\
        InceptionResnetV2 & 100\% \\
        InceptionV3 & 100\% \\
        InceptionV4 & 100\% \\
        LevitDistilled & 100\% \\
        Longformer & 100\% \\
        MNASNet & 36.36\% \\
        MlpMixer & 75.0\% \\
        MobileNetV2 & 75.0\% \\
        MobileNetV3 & 95.74\% \\
        MobileVIT & 100\% \\
        Nest & 100\% \\
        NormFreeNet & 95.65\% \\
        PoolingVisionTransformer & 100\% \\
        RegNet & 94.29\% \\
        RepVGG & 100\% \\
        Res2Net & 100\% \\
        ResNet & 92.94\% \\
        ResNetV2 & 92.59\% \\
        ResNext & 100\% \\
        RetinaNet & 100\% \\
        RexNet & 100\% \\
        RoBERTa & 88.89\% \\
        SENet & 90.48\% \\
        SK-ResNet & 100\% \\
        SK-ResNext & 100\% \\
        SeBotNet & 100\% \\
        SeResNet & 100\% \\
        SelecSls & 100\% \\
        ShuffleNetV2 & 100\% \\
        SqueezeBERT & 100\% \\
        SqueezeNet & 100\% \\
        SwinTransformer & 100\% \\
        SwinTransformerV2 & 100\% \\
        SwinTransformerV2Cr & 100\% \\
        Twins & 100\% \\
        VGG & 100\% \\
        Visformer & 100\% \\
        VisionTransformer & 84.85\% \\
        VisionTransformerDistilled & 100\% \\
        VisionTransformerRelPos & 71.43\% \\
        Xception & 100\% \\
        XceptionAligned & 100\% \\
        Xcit & 100\% \\
        Xmod & 100\% \\
\end{longtable}
